DensePoint: Learning Densely Contextual Representation for Efficient Point Cloud Processing

Point cloud processing is very challenging, as the diverse shapes formed by irregular points are often indistinguishable. A thorough grasp of the elusive shape requires sufficiently contextual semantic information, yet few works devote to this. Here we propose DensePoint, a general architecture to learn densely contextual representation for point cloud processing. Technically, it extends regular grid CNN to irregular point configuration by generalizing a convolution operator, which holds the permutation invariance of points, and achieves efficient inductive learning of local patterns. Architecturally, it finds inspiration from dense connection mode, to repeatedly aggregate multi-level and multi-scale semantics in a deep hierarchy. As a result, densely contextual information along with rich semantics, can be acquired by DensePoint in an organic manner, making it highly effective. Extensive experiments on challenging benchmarks across four tasks, as well as thorough model analysis, verify DensePoint achieves the state of the arts.

==> 3-method-recover1.tex <==
%how we achieve the two classic operations in CNN, \textit{i.e.}, convolution and pooling, on point cloud.
In this section, we first describe the generalized convolution along with pooling on point cloud. Then, we present DensePoint, and elaborate how it learns densely contextual representation for point cloud processing.

\subsection{Convolution and Pooling on Point Cloud}
\noindent\textbf{PConv: convolution on point cloud.} \
The classic convolution on image is operated on a local grid region, and the convolutional weight of this grid region is shared along the spatial dimension. However, this operation is difficult to achieve on point cloud due to the irregularity of points. To deal with this problem, we generalize the convolution on point cloud (PConv, for short) as
\begin{equation}
\label{Eq1:general_conv}
%{\bm{\mathrm f}}_{{\bm{\mathrm P}}_{c}} = \rho(\{\phi(x_j), \forall x_j \in \mathcal{N}(x_{i})\}), \ \ x_j \in \mathcal{N}(x_{i}) \ \text{if} \ d_{ij} < r,
{\bm{\mathrm f}}_{{\bm{\mathrm P}}_{c}} = \rho(\{\phi(x_j), \forall x_j \in \mathcal{N}(x_{i})\}), \ \ x_j \in \mathcal{N}(x_{i}) \ \text{if} \ d_{ij} < r,
\end{equation}
where ${\bm{\mathrm P}}_{c} \subset \mathbb{R}^3$, the local point cloud to convolute, is sampled from the whole point cloud by taking a sampled point $x_{i}$ as the centroid, and the nearby points as its neighbors $\mathcal{N}(x_{i})$. $d_{ij}$ is the 3D Euclidean distance between $x_{i}$ and $x_{j}$ and $r$ is the radius of this sphere neighborhood. Then $f_{{\bm{\mathrm P}}_{c}}$,
%gather function $\mathcal{G}$ on the transformed features with function $\mathcal{T}$ on all the points.
the convolutional result, is obtained by performing feature transformation on each point in ${\bm{\mathrm P}}_{c}$ with function $\phi$, and following a function $\rho$ to gather these transformed features. Finally, similar to the classic grid convolution, the feature of the centroid $x_i$ is updated with the learned single vector $f_{{\bm{\mathrm P}}_{c}}$, as an inductive representation of ${\bm{\mathrm P}}_{c}$.

In Eq. \eqref{Eq1:general_conv}, $f_{{\bm{\mathrm P}}_{c}}$ can be permutation invariant only when the inner function $\phi$ is shared over each point in ${\bm{\mathrm P}}_{c}$, and the outer function $\rho$ is symmetric (\textit{e.g.}, sum). Accordingly, for high efficiency, we employ a shared single-layer perceptron (SLP, for short), following a nonlinear activation function, as $\phi$ to implement feature transformation.
%and max pooling fully investigated in PointNet \cite{} as $\rho$ for gathering features with effectiveness (Fig. \ref{}). 
Meanwhile, as done in classic convolution, $\phi$ is also shared over each sampled local point cloud, for achieving the weight sharing mechanism. As a result, with a symmetric $\rho$, the generalized PConv can achieve efficient inductive learning of local patterns, whilst be independent of the irregularity of points. Further, using PConv as the basic operator, a classic CNN-like architecture, as shown in the upper part of Fig. \ref{fig2:DensePoint}, can be easily built with layer-by-layer connection.

Though efficient, PConv can be less effective for DensePoint, which will be clarified in Sec \ref{Sec:densepoint}. Therefore, we also present an enhanced PConv that are elaborated in Sec \ref{Sec:epconv}.

\noindent\textbf{PPool: pooling on point cloud.} \ 
In classic CNN, pooling is usually performed to explicitly raise the semantic level of the representation and improve computational efficiency. Here, using PConv, this operation can be achieved on point cloud in a learnable way. Specifically, $N_o$ points are first uniformly sampled from the input $N_i$ points, where $N_o < N_i$ (\textit{e.g.}, $N_o = N_i/2$). Then, PConv can be applied to pool all the local scopes centered on those sampled $N_o$ points.

%\subsection{Aggregately Learning Hierarchical Representation}
\subsection{Learning Densely Contextual Representation}
\noindent\textbf{Classic CNN architecture.} \
\label{Sec:normal_arch}
In classic CNN architecture with layer-by-layer connection (see the upper part of Fig. \ref{fig2:DensePoint}), hierarchical representations can be learned with the low-level ones in early layers and the high-level ones in deep layers \cite{deconv}. However, for this type of connection, a significant deficiency is, each layer can only learn from single-level representation. This results that all layers can capture only single-scale shape information from the input point cloud. Formally, assume a point cloud ${\bm{\mathrm P}}_{0}$ that is passed through this type of network. The network comprises $L$ layers, in which the $\ell^{th}$ layer performs a non-linear transformation $\mathcal{H}_{\ell}(\cdot)$. Then, the output of the $\ell^{th}$ layer can be learned from its previous layer as
\begin{equation}
\label{Eq2:layer_by_layer}
{\bm{\mathrm P}}_{\ell} = \mathcal{H}_{\ell}({\bm{\mathrm P}}_{\ell-1}),
\end{equation}
where ${\bm{\mathrm P}}_{\ell-1}$ is of single-scale receptive filed on the input point cloud ${\bm{\mathrm P}}_{0}$, resulting that each point in the learned ${\bm{\mathrm P}}_{\ell}$ captures only single-scale shape information. Finally, this will lead to a weakly contextual representation, which is not effective enough for identifying the diverse implicit shapes.
%for challenging point cloud processing.

\noindent\textbf{DensePoint architecture.} \ 
To mitigate the above deficiency, we present a general architecture, \textit{i.e.}, DensePoint as shown in the lower part of Fig. \ref{fig2:DensePoint}, inspired by dense connection mode \cite{densenet}. Specifically, for each layer in DensePoint, the outputs of all preceding layers are used as its input, and its own output is used as the input to all subsequent layers. That is, ${\bm{\mathrm P}}_{\ell}$ in Eq. \eqref{Eq2:layer_by_layer} becomes 
\label{Sec:densepoint}
\begin{equation}
\label{Eq3:dense_connect}
{\bm{\mathrm P}}_{\ell} = \mathcal{H}_{\ell}([{\bm{\mathrm P}}_{0}, {\bm{\mathrm P}}_{1}, \dots, {\bm{\mathrm P}}_{\ell-1}]),
\end{equation}
%where $[{\bm{\mathrm P}}_{0}, {\bm{\mathrm P}}_{1}, \dots, {\bm{\mathrm P}}_{\ell-1}]$ denotes the
where $[\cdot]$ denotes the concatenation of the outputs of all preceding layers. Here, ${\bm{\mathrm P}}_{\ell}$ is forced to learn from multi-level representations, which facilitates to aggregate multi-level shape semantics along with multi-scale shape information. In this organic way, each layer in DensePoint can capture a certain level (scale) of context, and the level can be gradually increased as the network deepens. Eventually, rich local-to-global shape information of the input ${\bm{\mathrm P}}_{0}$ can be \textit{progressively} aggregated together, resulting in a densely contextual representation for point cloud processing.

Note that DensePoint is quite different from traditional multi-scale strategy. The former progressively aggregates multi-level (multi-scale) semantics that are naturally learned by each layer, while the latter artlessly gathers multi-scale information at the same level. It is also dissimilar to simple concatenation of all layers as final output, which results that each layer fails to be contextual.

\noindent\textbf{Narrow architecture.} \
When the network deepens, DensePoint will suffer high complexity, since with all preceding layers as input, the convolutional overhead of deep layers will be huge. Thus, we narrow the output channels of each layer in DensePoint with a constant small number $k$ (\textit{e.g.}, 24), instead of the large ones (\textit{e.g.}, 512) in classic CNN.

\noindent\textbf{ePConv: enhanced PConv.} \ 
Though lightweight, such narrow DensePoint will lack the representational capacity, since with much narrow output $k$, the share SLP in PConv, \textit{i.e.}, $\phi$ in Eq. \eqref{Eq1:general_conv}, can be insufficient in learning ability. For a better representation, we introduce the grouping operation \cite{Alexnet} to enhance PConv. The enhanced PConv (ePConv, for short) converts Eq. \eqref{Eq1:general_conv} to 
\label{Sec:epconv}
\begin{equation}
%setlength{abovedisplayskip}{1pt}
%setlength{belowdisplayskip}{1pt}
\label{Eq4:enhance_conv}
f_{{\bm{\mathrm P}}_{c}} = \psi(\rho(\{\phi'(x_j), \forall x_j \in \mathcal{N}(x_{i})\})),
%\ \ x_j \in \mathcal{N}(x_{i}) \ \text{if} \ d_{ij} < r,
\end{equation}
where $\phi'$, the grouping version of SLP, can widen its output to enhance its learning ability and maintain the original efficiency, and $\psi$, an extra SLP (shared over each sampled centroid $x_i$), is added to integrate the detached information in all groups. Also, both $\phi'$ and $\psi$ follow a nonlinear activation function. To clarify, let SLP$^{\phi'}$ and SLP$^{\psi}$ denote the SLP of $\phi'$ and $\psi$ respectively, $C_i$ and $C_o$ denote the input channels and the output ones of SLP$^{\phi'}$ respectively, and $N_g$ denote the number of groups. Then, the parameter number of SLP$^{\phi'}$ before and after grouping is, $C_i \times C_o$ vs. $(C_i/N_g) \times (C_o/N_g) \times N_g = (C_i \times C_o)/N_g$. That is, $C_o$ can even be increased by $N_g$ times but results in the same complexity. Besides, inspired by the bottleneck layer \cite{resnet}, we fix the output channels of SLP$^{\phi'}$ and SLP$^{\psi}$ as $4k:k=4:1$, to hold the original narrowness for DensePoint. Thus, SLP$^{\psi}$ actually leads to only a little complexity with the small $k$, which can be easily remedied by suitable $N_g$.

\begin{figure}[t]
\centerline{\includegraphics[width=8.2cm]{figures/architecture/arch_cropped.pdf}}
\caption{Overview of the proposed relation-shape convolution.}
\label{fig3:arch}
\end{figure}

\begin{algorithm}[t]
\small
\caption{DensePoint algorithm}
\KwIn{point cloud ${\bm{\mathrm P}}$; input features \{$f_x, \forall x \in {\bm{\mathrm P}}$\}; depth $L$; weight matrices; non-linearity \sigma; }
\KwOut{$con(r_i)$}
$con(r_i)= \Phi$\;
\For{$j=1;j \le n;j \ne i$}
{
    float $maxSim=0$\;
    $r^{maxSim}=null$\;
    \While{not end of $T_j$}
    {
        compute Jaro($r_i,r_m$)($r_m\in T_j$)\;
        \If{$(Jaro(r_i,r_m) \ge \theta_r)\wedge (Jaro(r_i,r_m)\ge r^{maxSim})$}
        {
            replace $r^{maxSim}$ with $r_m$\;
        }
    }
    $con(r_i)=con(r_i)\cup {r^{maxSim}}$\;
}
return $con(r_i)$\;
\end{algorithm}

%{\renewcommand\baselinestretch{1}\selectfont
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}   %改成后面的小标题
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\renewcommand{\algorithmicrepeat}{\textbf{Repeat:}}   %改成后面的小标题
%\renewcommand{\algorithmicuntil}{\textbf{Until:}}
%\renewcommand{\algorithmicreturn}{\textbf{Return:}}
%\begin{algorithm}[t]
%\caption{\ Training and Test of S-Cls model}
%\label{alg:train_test}
%%\small
%%\footnotesize
%\begin{algorithmic}[1]
%\TRAINING ~~ \\
%\REQUIRE image data and label data $(\mathbf{I}^N,y^N)$.
%%, where $y\in\{1,\cdots,K\}$, $i\in\{1,\cdots,M\}$ and $j\in\{1,\cdots,N\}$
%\ENSURE parameters $\mathbf{w}$ of S-Cls model.
%\INITIALIZE $\mathbf{w}$, $\lambda$ and training hyper-parameters.
%\STAGEONE Feature-Level Knowledge Transfer.
%\REPEAT
%\STATE compute ${\bm L}_f ({\mathbf w}_{\rm conv}^{\mathcal{S}})$ by Eq. (\ref{Eq:loss_featureLevel}), Eq. (\ref{Eq:roi_feature}).
%\STATE update ${\mathbf w}_{\rm conv}^{\mathcal{S}}$ by gradient back-propagation.
%\UNTIL ${\bm L}_f ({\mathbf w}_{\rm conv}^{\mathcal{S}})$ converges.
%\STAGETWO Prediction-Level Knowledge Transfer.
%\REPEAT
%\STATE compute ${\bm L}_{p}({\mathbf w}^{\mathcal{S}}) + {\lambda} {\bm L}_{p'}({\mathbf w}^{\mathcal{S}})$ by Eq. (\ref{Eq:loss_soft}), Eq. (\ref{Eq:loss_hard}), Eq. (\ref{Eq:loss_all}).
%\STATE update ${\mathbf w}^{\mathcal{S}}$ by gradient back-propagation.
%\UNTIL ${\bm L}_{p}({\mathbf w}^{\mathcal{S}})$ converges.
%\MYRETURN ${\mathbf w}^{\mathcal{S}}$
%%\item[]
%\vspace{+1mm}
%\TESTING ~~ \\
%\REQUIRE image data $\mathbf{I}^N$.
%\ENSURE prediction $l^N$.
%\INITIALIZE parameters $\mathbf{w}$ of S-Cls model, confidence threshold $\tau$.
%\FOR {$n=1$ to $N$}
%\STATE forward pass S-Cls model to get $p(\mathbf{I}^n|{\mathbf w})$.
%\STATE compute $l^n$ by Eq. (\ref{Eq:problem_formula}).
%\ENDFOR
%\MYRETURN $l^N$
%\end{algorithmic}
%\end{algorithm}
%\par} %最后这句是取消后面语句的算法格式，使其恢复先前的格式

\noindent\textbf{DensePoint for point cloud processing.} \ 


\noindent\textbf{Implementation details.} \
For convolutional layers (Eq. \eqref{Eq4:enhance_conv}), inspired by pre-activation \cite{eccv16:identity mapping}, $H_{\ell}(\cdot)$ is defined as a sequential composite operation of Batch Normalization (BN) \cite{} $\to$ Rectified Linear Units (ReLU) \cite{} $\to$ SLP$^{\phi'}$ $\to$ BN $\to$ ReLU $\to$ Max pooling $\rho$ $\to$ SLP$^{\psi}$. Similarly, for pooling layers (Eq. \eqref{Eq1:general_conv}), $H_{\ell}(\cdot)$ is defined as SLP$^{\phi}$ $\to$ BN $\to$ ReLU $\to$ Max pooling $\rho$. The network of DensePoint comprises 14 layers: \textit{Input($C$ channels, $N$ points) $\to$ Pooling($C$, 96, $N/2$) $\to$ 3$\times$E-PConv(k=24, $N/2$) $\to$ Pooling(168, 144, $N/4$) $\to$ 5$\times$E-PConv(k=36, $N/4$) $\to$ Pooling(324, 512, 1) $\to$ fc(512, 256, class number)}, . The first 11 layers , while the last 3 layers


